On forest-type tree ensemble approaches to density learning under a generalized Bayesian framework

We study density forests (DFs), a class of forest-type tree ensembles designed for multivariate density learning. A DF is an aggregation of tree base learners for density functions, each growing under a small perturbation of the original data. We investigate the bias-variance trade-off of DFs and introduce Bayesian and generalized Bayesian strategies to enhance the data adaptivity of DFs, called Bayesian density forests (BDFs) and Gibbs density forests (GDFs), respectively. The BDF improves the data adaptivity of DFs by aggregating forests of varying depths with respect to the marginal posterior distribution on tree depth. The GDF, on the other hand, employs an empirical risk function for each forest topology and makes risk-based generalized Bayesian inference through the resulting Gibbs posterior to learn the forest topology from the data, thereby overcoming limitations of the likelihood in effectively quantifying the bias-variance trade-off for tree ensembles. For both BDF and GDF, we analyze their asymptotic properties, demonstrating that these ensembles can achieve faster convergence compared to single tree-based approaches for estimating smooth density functions. The GDF exhibits superior data adaptivity, achieving the minimax convergence rate up to a logarithmic term over anisotropic H\"older spaces with varying smoothness levels along different dimensions. We identify a set of conditions ensuring fast posterior contraction of GDFs in more general settings. Moreover, we provide empirical risk bounds that clarify the bias-variance decomposition for individual trees and forest-type ensembles in the density learning context. We propose efficient computational algorithms for computing the density estimates under BDF and GDF and illustrate the practical performance of these methods through simulations in both low-dimensional and moderately high-dimensional settings.

==> BMAposterior/forestpenalty.tex <==
\subsection{Imposing regularization for forests}

\subsubsection{Random subsampling of variables}
Assume at each step, $m$ features are randomly selected for splitting. Then for each tree, at each step, the probability of randomly selecting a feature $X_1$ for splitting is
\begin{eqnarray*}
  \frac{\binom{d-1}{m-1}}{\binom{d}{m}} = \frac{(d-1)! m! (d-m)!}{d! (m-1)! (d-m)!} = \frac{m}{d}.
\end{eqnarray*}
If a tree is of depth $k$, then the probability that $X_1$ is not sampled for splitting in this tree is 
\begin{eqnarray*}
  \l 1 - \frac{m}{d} \r^k.
% = 1 - k \cdot \frac{m}{d} + \frac{1}{2} k (k-1) \l \frac{m}{d} \r^2.
\end{eqnarray*}
The probability of the opposite event is 
\begin{eqnarray*}
  1 - \l 1 - \frac{m}{d} \r^k .
%\approx \frac{k m}{d}.
\end{eqnarray*}

\subsubsection{Regularization for forests}
In order to achieve adaptivity, we need to have a reasonably well estimation of 
\begin{eqnarray*}
  K(f_0, f_k^\en) = \E_{f_0} \l \log \frac{f_0(Y)}{f_k^\en (Y)} \r.
\end{eqnarray*}

A natural estimation of this quantity is 
\begin{eqnarray*}
  \frac{1}{n} \sum_{i=1}^n \log \frac{f_0(Y_i)}{\hat{f}_k^\en (Y_i)}.
\end{eqnarray*}
Note that
\begin{eqnarray*}
   \frac{1}{n} \sum_{i=1}^n \log \frac{f_0(Y_i)}{\hat{f}_k^\en (Y_i)}
&=& 
\frac{1}{n} \sum_{i=1}^n 
\l 
\log \frac{f_0(Y_i)}{{f}_k^\en (Y_i)}
+ \log \frac{f_k^\en(Y_i)}{\hat{f}_k^\en (Y_i)} 
\r \\
&=& 
\frac{1}{n} \sum_{i=1}^n 
\log \frac{f_0(Y_i)}{{f}_k^\en (Y_i)}
- \frac{1}{n}  \sum_{i=1}^n \log \frac{\hat{f}_k^\en(Y_i)}{{f}_k^\en (Y_i)}.
\end{eqnarray*}
For the second part in the last equation, more explicitly,
\begin{eqnarray*}
  - \frac{1}{n}  \sum_{i=1}^n \log \frac{\hat{f}_k^\en(Y_i)}{{f}_k^\en (Y_i)}
&=& -\frac{1}{n}  \sum_{i=1}^n \log 
\l \frac{1}{B} \sum_{b=1}^B \frac{\hat{f}_k^\bsup (Y_i)}{{f}_k^\en (Y_i)}
\r.
\end{eqnarray*}

For the upper bound, based on the concavity of the logarithm function, 
\begin{eqnarray*}
  - \frac{1}{n} \sum_{i=1}^n \log \frac{\hat{f}_k^\en(Y_i)}{{f}_k^\en (Y_i)}
&\leq& - \sum_{i=1}^n \frac{1}{B} \sum_{b=1}^B 
\log \frac{\hat{f}_k^\bsup (Y_i)}{{f}_k^\en (Y_i)} \\
&=&  \frac{1}{B} \sum_{b=1}^B  \frac{1}{n} \sum_{i=1}^n 
\l 
-\log \frac{\hat{f}_k^\bsup (Y_i)}{{f}_k^\en (Y_i)} 
\r.
\end{eqnarray*}
By applying the inequality (\ref{eq:OneSideIneqLower}), or based on the definition of the MLE, we can obtain an upper bound of this term. In particular, we should be able to show that 
\tech{
  \begin{eqnarray*}
     - \frac{1}{n} \sum_{i=1}^n \log \frac{\hat{f}_k^\en(Y_i)}{{f}_k^\en (Y_i)}
\leq 
\frac{\eta' t \log t \log n}{n},
  \end{eqnarray*}
with probability tending to 1. 
}
Combining the bound together, we have 
\begin{eqnarray*}
  - \sum_{i=1}^n \log \hat{f}_k^\en (Y_i) + \sum_{i=1}^n \log f_0(Y_i) 
\leq \sum_{i=1}^n \log  \frac{f_0(Y_i)}{{f}_k^\en (Y_i)} + \eta' t \log t \log n.
\end{eqnarray*}
It is fine to replace the sample mean by the expectation, as it converges very fast, at root $n$ rate. 
\begin{eqnarray*}
  - \sum_{i=1}^n \log \hat{f}_k^\en (Y_i) +  n \int f_0 \log f_0 
\leq n K (f_0, {f}_k^\en)+ \eta' t \log t \log n.
\end{eqnarray*}

\tech{For the lower bounded, a trick that will be applied is, for nonnegative numbers $a, b, c$,
 and $d$, we have
 \begin{eqnarray*}
\min \left\{ \frac{a}{c}, \frac{b}{d} \right\}
\leq
   \frac{a+b}{c+d}
   \leq
   \frac{a}{c}
   + \frac{b}{d}.
 \end{eqnarray*}
 Then,
  \begin{eqnarray*}
     - \frac{1}{n}  \sum_{i=1}^n \log \frac{\hat{f}_k^\en(Y_i)}{{f}_k^\en (Y_i)}
    &=&
        - \frac{1}{n}  \sum_{i=1}^n \log
        \frac{\sum_{b=1}^B \hat{f}_k^\bsup (Y_i)}
        {\sum_{b=1}^B {f}_k^\bsup (Y_i)}  \\
    &\geq&
      - \frac{1}{n}  \sum_{i=1}^n \log
           \l
          \sum_{b=1}^B \frac{\hat{f}_k^\bsup (Y_i)}
           {{f}_k^\bsup (Y_i)}
           \r\\
     &=&
      - \frac{1}{n}  \sum_{i=1}^n \log
           \frac{1}{B} \l
          \sum_{b=1}^B \frac{\hat{f}_k^\bsup (Y_i)}
           {{f}_k^\bsup (Y_i)}
           \r - \log B.
  \end{eqnarray*}
 }

\tech{One way to derive the lower bound is by assuming both the true density and the estimate are bounded from the above and below. If this is the case, then even the logarithm function is concave, we can still find a constant $\tau>1$, such that
  \begin{eqnarray*}
     - \frac{1}{n}  \sum_{i=1}^n \log
           \frac{1}{B} \l
          \sum_{b=1}^B \frac{\hat{f}_k^\bsup (Y_i)}
           {{f}_k^\bsup (Y_i)}
           \r 
 &\geq & - \tau \sum_{i=1}^n \frac{1}{B} \sum_{b=1}^B 
\log \frac{\hat{f}_k^\bsup (Y_i)}
           {{f}_k^\bsup (Y_i)}\\
&=&  \frac{\tau}{B} \sum_{b=1}^B  \frac{1}{n} \sum_{i=1}^n 
\l 
-\log \frac{\hat{f}_k^\bsup (Y_i)}
           {{f}_k^\bsup (Y_i)}
\r.
  \end{eqnarray*}
Then a lower bound can be derived by applying the inequality (\ref{eq:OneSideIneqUpper}). With a similar argument, we have 
\begin{eqnarray*}
  - \sum_{i=1}^n \log \hat{f}_k^\en (Y_i) +  n \int f_0 \log f_0 
\geq n K (f_0, {f}_k^\en) - \tau \eta t \log t \log n.
\end{eqnarray*}
}

==> GibbsPosterior/shape.tex <==
\subsection{Posterior Concentration Under Shape Constraints}

First, we will show that if a tree is grown under shape
constraints, then the posterior distribution will concentrate around
the ``best'' approximation supported by the constrained tree
topology.
We would like to exactly quantify how fast this concentration is. The
result is summarized in the following theorem. 
% Although the posterior may not concentrate at the optimal rate, it
% even may not be consistent, we will try to argue that this is mainly
% due to the poor approximation ability, or the bias. The variance
% component is still under control.
\begin{theorem}
  Assume $f_0 \in H^{\bm \alpha}$, $\alpha_l \in (0, 2]$. Let $\overline{\alpha} = \left( \frac{1}{d} \sum_{l=1}^d \alpha^{-1}\right)^{-1}$. Under a shape constrained OPT prior with tree topology within the
  equivalence class $\wt{\A}_{\bm k}$, when
  $$\sum_{l=1}^d k_l \leq  \Big ( n/ \log n \Big)^{\frac{1}{2 \alpha}}$$
\end{theorem}

==> partition_select/variance_forest_rev.tex <==
\rev{\subsubsection{Estimation error}
\begin{theorem}
   \label{thm:var_deviation}
  Given a partition $\mathcal{A}_t = \{\Omega_j\}_{j=1}^t$ of size $t$, either with or without the shift, we define the ``projection'' of the true density function onto the partition as
  \begin{eqnarray*}
   f_{\mathcal{A}_t}= \sum_{j=1}^t \frac{\theta_j}{\mu(\Omega_j)}  \cdot \mathbbm{1}_{\Omega_j}, \quad \mbox{with } \theta_j = \int_{\Omega_j}f_0.
  \end{eqnarray*}
  and the maximum likelihood estimator supported by the partition
  $\mathcal{A}_t$ is denoted as $\hat{f}_{n, \mathcal{A}_t}$. Let $\delta_{n, t} = \left( \frac{t \log t }{n / \log
    n} \right) ^{1/2}$, where $t = O(n^{\frac{1}{2r+1}})$ for some $r>0$. \tech{Under
  conditions 1-3}, for $\eta>1$ and some $c_2 \in (0, 1)$, we have
  \begin{eqnarray}
    \label{eq:var_deviation}
    \P_0^n \left( \rho (\hat{f}_{n, \mathcal{A}_t}, f_{\mathcal{A}_t}) \geq
    \eta \delta_{n, t} \right) \leq 4 \exp(-c_2 \eta^2 n \delta_{n, t}^2 ),
  \end{eqnarray}
  and
  \begin{eqnarray}
    \label{eq:var_deviation_lik}
    \P_{f_0} \left( \sup_{f \in \mathcal{F}_{\mathcal{A}_t} } \prod_{i=1}^n
    \frac{f(Y_i)}{\fat(Y_i)} \geq \exp( \eta^2 n \delta_{n, t}^2)
    \right)
    \leq
    8\exp(-c_2 \eta^2 n \delta_{n, t}^2 ).
  \end{eqnarray}
\end{theorem}}

\rev{The result can be obtained by applying the one-sided large deviation
inequality iteratively. Before providing more details of the proof, we
would like to introduce a truncated version of the likehood ratio,
when the true density $f_0$ is replaced by the ``best approximation''
$f_{\mathcal{A}_t}$ within $\mathcal{F}_{\mathcal{A}_t}$.
Let $Z_{\mathcal{A}_t, f} (Y_i) = \log 
(f(Y_i) /f_{\mathcal{A}_t}(Y_i))$. The lower-truncated versions of $f$
and $Z_{\mathcal{A}_t, f}$ are defined similarly as before,
\begin{eqnarray*}
  \tilde{f} =
  \begin{cases}
    f, & \mbox{if } f > \exp(-\tau) f_{\mathcal{A}_t}, \\
    \exp(-\tau) f_{\mathcal{A}_t}, & \mbox{if } f \leq \exp(-\tau) \fat.
  \end{cases}\\
                                     \widetilde{Z}_{\at, f } = Z_{\at, \tilde{f}} =
  \begin{cases}
    Z_{\at, f}, & \mbox{if } Z_{\at, f} > - \tau, \\
    -\tau, & \mbox{if } Z_{\at, f} \leq -\tau. 
  \end{cases}
\end{eqnarray*}
\techrev{We can show that, the likelihood ratio with respect to
  $\fat$ still enjoys most desired properties. In particular, Lemma \ref{lemma:boundofexpectation} and Lemma
  \ref{lemma:largedeviation} still holds if we replace $f_0$ by
  $\fat$. Without checking the proofs for those two lemmas, we can
  verify this point by the following ``change-of-measure'' type
  argument: given the partition, the approximating space can be
  viewed as a collection of multinomial distributions. The sufficient
  statistics for this model is the vector of counts $(\sum_{i=1}^n
  \mathbbm{1}_{X_i \in \Omega_j})_{1 \leq j \leq t}$. The distribution
of the random vector remains the same if we view the data as they are generated
from $\fat$. This implies that, in Lemma \ref{lemma:boundofexpectation} and Lemma
  \ref{lemma:largedeviation}, the probability of the events envolved
  in the proof is the same as that measured under
  $\fat$. Therefore, results can be obtained by treating $\fat$ as the
  true distribution.  }}
\begin{proof}
  % When the partition is fixed, a useful observation is if the MLE is
%   known to be contained in a set $\mathcal{C} \subset \fat $, then 
%     \begin{eqnarray*}
%     K\l(\hat{f}_{n,\mathcal{A}_t}, f_{\mathcal{A}_t}  \r) 
% &=& \int \hat{f}_{n, \mathcal{A}_t} \log \frac{\hat{f}_{n, \mathcal{A}_t}}{ f_{\mathcal{A}_t} }\\
% &=& \sum_{j=1}^t \frac{n_j}{n}
%     \log \frac{n_j/n}{\theta_j} \\
% &\leq& 
% \sup_{f \in \mathcal{C}} 
%  \frac{1}{n} \sum_{i=1}^n \log\left(  f(Y_i) / f_{\mathcal{A}_t} (Y_i) \right).
%     \end{eqnarray*}
\rev{In the proof, Lemma \ref{lemma:largedeviation} will be applied iteratively to
obtain a ``sharp'' bound of $ \rho \l(\hat{f}_{n,\mathcal{A}_t},
f_{\mathcal{A}_t}  \r)$. Let $\delta_k(n, t) = \left(\frac{t \log t}{n
    / \log n} \right)^{\omega_k}$, where $\omega_k$ is a
sequence defined by 
\begin{eqnarray}
  \label{eq:omega}
 \omega_1= 1/4 \quad \mbox{and} \quad \omega_{k+1} = \frac{1}{2}
\omega_k + \frac{1}{4}.
\end{eqnarray}
We also define $\C_1:= \{ f \in \mathcal{F}_\at: \rho (f, \fat) \geq
\eta \delta_1(n,
t) \}$ and $\C_k := \{ f \in \mathcal{F}_\at: \eta \delta_k(n,t) \leq
\rho (f, \fat) < \eta \delta_{k-1}(n,t) \}$ for $k\geq 2$.}

\rev{When $k=1$, by definition of the MLE, we have 
\begin{eqnarray}
\label{eq:DistToRatio}
\nonumber  \mathbb{P}_0^n \left( \rho ( \hat{f}_{n, \at}, f_\at ) \geq \eta
  \delta_1(n,t) \right) 
&\leq& 
\mathbb{P}_{f_0} \left( \sup_{f \in \mathcal{C}_1 } L_n(f) \geq \sup_{f \in
  \mathcal{F}_\at} L_n(f) \right)\\
&\leq& 
\mathbb{P}_{f_0} \left( \sup_{f \in \C_1} L_n (f) \geq
  L_n (f_\at) \right).
\end{eqnarray}
By applying the lower truncation of the log-likelihood ratio, the
above probability can be further bounded by 
\begin{eqnarray}
\label{eq:toLowerTrunc}
  \mathbb{P}_0^n \left( \rho ( \hat{f}_{n, \at}, f_\at ) \geq \eta
  \delta_1(n,t) \right) 
\leq \mathbb{P}_{f_0} \left( \sup_{f \in \C_1} \sum_{i=1}^n
\widetilde{Z}_{\at, f} (Y_i) \geq 0 \right).
\end{eqnarray}
Note that the modified version of Lemma \ref{lemma:boundofexpectation}
can still be applied to $\widetilde{Z}_{\at, f}$, which implies that 
\begin{eqnarray*}
  \sup_{f \in \C_1} \left( - \E  \widetilde{Z}_{\at, f} (Y_1 )\right) \geq (1
  -\gamma) \rho^2( f, \fat),
\end{eqnarray*}
Together with previous upper bound (\ref{eq:toLowerTrunc}), we obtain 
\begin{eqnarray}
\label{eq:toEP}
  \nonumber && \mathbb{P}_0^n \left( \rho ( \hat{f}_{n, \at}, f_\at ) \geq \eta
  \delta_1(n,t) \right)  \\
\nonumber  && \hspace{1cm} \leq  
\mathbb{P}_{f_0} \left( \sup_{f \in \C_1} n^{-1/2}
\sum_{i=1}^n 
\left(\widetilde{Z}_{\at, f} (Y_i) 
- \mathbb{E} \widetilde{Z}_{\at, f} (Y_i ) \right) 
\geq
-n^{-1/2} \sum_{i=1}^n 
\sup_{f \in \C_1} \left(\mathbb{E} \widetilde{Z}_{\at, f} (Y_i)
\right) \right)\\
&& \hspace{1cm} \leq
\mathbb{P}_{f_0} \left( \sup_{f \in \C_1} n^{-1/2}
\sum_{i=1}^n \left(\widetilde{Z}_{\at, f} (Y_i ) - \mathbb{E}
   \widetilde{Z}_{\at, f} (Y_i ) \right) \geq
n^{1/2} (1-\gamma) \eta^2 \delta_1^2(n, t) \right).
\end{eqnarray}
In order to apply Lemma \ref{lemma:largedeviation} to bound the
probability on the right hand side of inequality (\ref{eq:toEP}), we need to check the conditions
(\ref{eq:condition1}) and (\ref{eq:condition2}). Note that $ \| f^{1/2} - f_\at ^{1/2} \|_2 ^2 = 2-2 \int_{\Omega}
\sqrt{f(y) f_\at (y) } dy \leq 2$. We may set $d$ in Lemma
\ref{lemma:largedeviation} to be 2 here. When $ t \sim
n^{\frac{1}{2r+1}}$, 
$\delta_1(n, t)= (\frac{t \log t} {n/ \log n})^{1/4}$ converges to zero as $n, t
\rightarrow \infty$. $L$ in Lemma \ref{lemma:largedeviation} is $n^{1/2}
(1-\gamma) \eta^2 \delta_1^2(n,t)$ here. First (\ref{eq:condition1}) is satisfied, since
\begin{equation*}
  L = n^{1/2} (1-\gamma) \eta^2 \delta_1^2(n,t) = o\left(b n^{1/2}
 d^2/4 \right). 
\end{equation*}
By observing $\mathcal{F}_\at
\subset \mathcal{F}_t$, for the function class $\mathcal{F}_\at$ we can use the same bound for the bracketing
entropy as that in Lemma
\ref{lemma:dballupperbound}. Even it seems to be a slightly loose
upper bound, it is still sufficient for our analysis of the estimation
error. By carrying out similar calculation as that for Lemma
\ref{cor:largedeviation},
\begin{eqnarray*}
 \int_{\frac{b (1-\gamma)}{32} \eta^2 \delta_1^2(n,t)}^d \left( \bentro ( u/(2 \exp{\tau/2}),
  \mathcal{F}_\at, \rho) \right)^{1/2} du  
\lesssim \sqrt{t \log t}.
\end{eqnarray*}
Therefore, (\ref{eq:condition2}) is also satisfied when $n$ and $t$
are large enough. With Lemma \ref{lemma:largedeviation}, we have
\begin{eqnarray}
  \label{eq:largedevf_I}
 \nonumber \mathbb{P}_0^n \left( \rho( \hat{f}_{n,t}, f_\at) > \eta
  \delta_1(n,t) \right)
&\leq& 3\exp
  \left(-(1-b) \varphi(L, d^2, n) \right) \\
&\leq&3 \exp\left( -\frac{(1-b) (1-\gamma)^2 \eta^2}{2^8 c_0 + 8}
       \cdot t (\log t) (\log n) \right).
\end{eqnarray}}

\rev{When $k\geq 2$, we still want to apply Lemma
\ref{lemma:largedeviation} to establish the inequality
\begin{eqnarray}
  \label{eq:largedevCm}
  \nonumber & &\mathbb{P}_0^n \left(\eta \delta_k(n,t) \leq \rho( \hat{f}_{n,\at},  f_\at) < \eta \delta_{k-1}(n,t) \right) \\
&\leq& 3 \exp\left( -\frac{(1-b) (1-\gamma)^2 \eta^2}{2^8 c_0 + 8}
       \cdot t (\log t)
(\log n) \right).
\end{eqnarray}
To do so, at the first step, by a similar argument as that for
inequalities (\ref{eq:DistToRatio}), (\ref{eq:toLowerTrunc}) and
(\ref{eq:toEP}), we have 
\begin{eqnarray}
  \label{eq:Cmeq1}
 \nonumber & &\mathbb{P}_0^n \left(\eta \delta_k(n,t) \leq \rho( \hat{f}_{n,\at},  f_\at) < \eta \delta_{k-1}(n,t) \right) \\
&&\hspace{0.8cm} \leq \mathbb{P}_{f_0} \left( \sup_{f \in \C_k} n^{-1/2} \sum_{i=1}^n
\left(\widetilde{Z}_{\at, f}(Y_i) - \mathbb{E} \widetilde{Z}_{\at, f} (Y_j) \right) \geq
n^{1/2}(1-\gamma) \eta^2 \delta_k^2(n,t) \right).
\end{eqnarray}
Now $L$ in Lemma \ref{lemma:largedeviation} is $n^{1/2}(1-\gamma) \eta^2
\delta_k^2(n,t)$ here and $d$ can be set as $\eta \delta_{k-1}(n,t)$. By our assumptions, $\delta_k(n,t) = o(\delta_{k-1}(n,t))$ for $k\geq
2$. Then condition (\ref{eq:condition1}) is satisfied.
Based on the same type of calculation,
\begin{eqnarray*}
  & &\int_{\frac{b (1-\gamma)}{32} \eta^2
    \delta_k^2(n,t)}^{\eta \delta_{k-1}(n,t)} \left( \bentro ( u/(2 \exp{\tau/2}),
  \mathcal{F}_\at, \rho) \right)^{1/2} du \\
&& \hspace{1cm} \lesssim t^{1/2} ( \eta \delta_{k-1}(n,t) \sqrt{ \log
  \frac{t^2}{\eta \delta_{k-1}(n,t)}} -\beta \delta^2_k(n,t) \sqrt{\log
  \frac{t^2}{\beta \delta_k^2(n,t)}}\\
& & \hspace{2cm}+ \frac{\sqrt{\pi}}{2} t^2 (
\frac{ \frac{\eta \delta_{k-1}(n,t)}{t^2} }{\sqrt{\pi \log
    \frac{t^2}{\eta \delta_{k-1}(n,t)}}} - \frac{ \frac{\beta \delta_k^2(n,t)}{t^2} }{\sqrt{\pi \log
    \frac{t^2}{\beta \delta_k^2(n,t)}}} ) )  \\
&& \hspace{1cm} \asymp t^{1/2} \delta_{k-1}(n,t) \sqrt{\log \frac{t^2}{\delta_{k-1}(n,t)}},
\end{eqnarray*}
where $\beta = \frac{b (1-\gamma)}{32} \eta^2 $. Plugging in $\delta_{k-1}(n,t) = (\frac{t
  \log t}{n/ \log n})^{\omega_{k-1}}$, after some calculation, we can
verify that condition (\ref{eq:condition2}) is also satisfied when
$n$ and $t$ are large enough.
Note that 
\begin{eqnarray*}
 & & \hspace{-1.5cm} \varphi(n^{1/2}(1-\gamma) \eta^2
\delta_k^2(n,t), (\eta \delta_{k-1}(n,t))^2, n) \\
&=& \frac{n(1-\gamma)^2 \eta^4
\delta_k^4(n,t)} {8(8c_0 \eta^2 \delta_{k-1}^2(n,t) +(1-\gamma)\eta^2
\delta^2_k(n,t))}\\
&\geq& \frac{n(1-\gamma)^2 \eta^2
\delta_k^4(n,t)} {8(8c_0 \delta_{k-1}^2(n,t) +(1-\gamma)
\delta^2_{k-1}(n,t))} \\
&\geq& \frac{n(1-\gamma)^2 \eta^2
(\frac{t \log t}{n / \log n})^{2\omega_{k-1}+1}} {(2^8 c_0 +8(1-\gamma))
(\frac{t \log t}{n/ \log n})^{2\omega_{k-1}}} \\
&\geq& \frac{(1-\gamma)^2 \eta^2 }{2^8 c_0 + 8} \cdot t (\log t) (\log n).
\end{eqnarray*}
Applying Lemma \ref{lemma:largedeviation}, we get the inequality
(\ref{eq:largedevCm}).}

\rev{Based on (\ref{eq:omega}), it is easy to see $\omega_k = \frac{1}{2}-
\( \frac{1}{2} \)^{k+1}$. % Condition (\ref{eq:thmC2}) assumes that
% $\frac{t \log t}{n /\log n} =
% o(1)$.
If we set $K(n,t)$ to be $\frac{\log \log \frac{n/\log n}{t \log
    t} - \log \log c}{\log c}$, then $\eta \delta_{K(n,t)} \leq c\eta
\delta_{n,t}$. It implies that 
\begin{eqnarray*}
 & &\mathbb{P}_0^n \left(\rho (\hat{f}_{n, \at}, f_\at) \geq c \eta \delta_{n,t} \right) \\
&&\hspace{1cm} \leq \mathbb{P} \left(\rho(\hat{f}_{n,\at}, f_\at) \geq \eta
\delta_1(n,I) \right) \\
& & \hspace{2cm} + \sum_{k=2}^{K(n,t)} \mathbb{P}_0^n \left(\eta \delta_k (n,t) \leq
\rho(\hat{f}_{n, \at}, f_\at) < \eta \delta_{k-1}(n,t) \right) \\
&&\hspace{1cm} \leq 3 K(n,t) \exp\left( -\frac{(1-b) (1-\gamma)^2
   \eta^2}{2^8 c_0 + 8} \cdot 
t (\log t) (\log n) \right).
\end{eqnarray*}
Therefore, for some $\eta>1$ and appropriately chosen $c_2$, the
inequality (\ref{eq:var_deviation}) holds.}

\rev{The proof for (\ref{eq:var_deviation_lik}) is similar.}

 % Based on this, we have  
%   \begin{eqnarray*}
%    && \mathbb{P} \left(  K\l(\hat{f}_{n,\mathcal{A}_t}, f_{\mathcal{A}_t}  \r)   \geq
%        \eta n \delta_{n, t}^2   \right) 
% \\ && \hspace{1cm} \leq \mathbb{P}_{f_0} \left( \sup_{f \in \mathcal{F}_\at } 
%  \sum_{i=1}^n \log\left( f/ f_{\mathcal{A}_t}  \right) (Y_i) 
%       \geq \eta n \delta_{n, t}^2 \right). \\
%  && \hspace{1cm} \leq \mathbb{P}_{f_0} \left( \sup_{f \in
%     \mathcal{F}_\at }
%     \sum_{i=1}^n
%     \widetilde{Z}_{\at, f}(Y_i) \geq \eta n \delta_{n, t}^2  \right)\\
% && \hspace{1cm} \leq  \mathbb{P}_{f_0} \left( \sup_{f \in\mathcal{F}_\at }
%  \sum_{i=1}^n \left( \widetilde{Z}_{\at, f}(Y_i)  
% - \mathbb{E} \widetilde{Z}_{\at, f}(Y_i) \right) 
% \geq \eta n  \delta_{n, t}^2 
% -n \sup_{f \in \mathcal{F}_\at} \mathbb{E} \widetilde{Z}_{\at, f}(Y_1)
%    \right) \\
%     && \hspace{1cm} \leq  \mathbb{P}_{f_0} \left( \sup_{f \in\mathcal{F}_\at }
%   n^{-1/2}\sum_{i=1}^n \left( \widetilde{Z}_{\at, f}(Y_i)  
% - \mathbb{E} \widetilde{Z}_{\at, f}(Y_i) \right) 
% \geq \eta n^{1/2}  \delta_{n, t}^2 
%    \right),
%  \end{eqnarray*}
% where the last inequality is obtained by applying the modified version
% of Lemma \ref{lemma:boundofexpectation}. That is, we have $-
% \mathbb{E} \widetilde{Z}_{\at, f}(Y_1) \geq (1- \gamma) \| f^{1/2} -
% \fat^{1/2}\|_2^2 \geq 0.$

% As the partition for $f_t^\m$ is exactly $\{ \Omega_j^\m \}_{j=1}^t$,
% $\mathbb{E} \log\left( f/ f_t^\m \right) (Y_1)  = - K(f_t^\m, f) $ for
% $f$ supported by the same partition. This implies 
% \begin{eqnarray*}
%   P_m \leq \mathbb{P}_{f_0} \left( \sup_{f \in \mathcal{F}(\{ \Omega_j^\m \}_{j=1}^t ) } 
%  n^{-1/2} \sum_{i=1}^n \left( \log\left( f/ f_t^\m \right) (Y_i)  
% - \mathbb{E} \log\left( f/ f_t^\m \right) (Y_i) \right) 
% \geq n^{1/2} \eta t \log t/n  \right).
% \end{eqnarray*}
\end{proof}

==> polya_tree/priorupper.tex <==
\subsection{Decay of the OPT Prior as the Depth Increases}
We would also like to obtain an upper bound of the prior probability mass on a random measure $f$ supported by a binary partition with $t$ subregions.
In particular, we wish to obtain an upper bound in the following form,
\begin{eqnarray}
  \label{eq:priorupperbound}
  \Pi \l \Theta_t \r \leq \exp(- \lambda t \log t ) \quad \mbox{for some } \lambda >0. 
\end{eqnarray}
For and $f \in \Theta_t$, define the depth of a binary partition (or a tree) as
\begin{eqnarray*}
  \D(\at) = \max \{ k: \at \cap \mathcal{R}^\ksup \neq \emptyset. \}
\end{eqnarray*}
%To simplify the notation, we may also write the depth as $\D$ when there is only one binary partition under discussion.
Assume the binary partition $\at$ is generated by a specific path $\mathcal{A}_t^\1, \mathcal{A}_t^\2, \ldots, \mathcal{A}_t^{(\D)}$,  where each $\A_t^\ksup, 1
\leq k \leq \D $ is a binary partition obtained after $k$ steps of
recursive partitioning.  The random measures supported by $\A_t$ grown
in this specific way is denoted as $\F_{\treea}$.

\subsubsection{A balanced partition is preferred}
For any two binary partitions $\A_{t}$ and  $\B_t$ of depths $\D_a$ and $\D_b$ respectively, we claim that
\begin{eqnarray}
  \label{eq:preferbal}
  \Pi \l \F_{\treea} \r \geq \Pi \l \F_{\treeb} \r \quad \mbox{if} \quad \D_a < \D_b. 
\end{eqnarray}

The proof is based on the observation that when we prune a pair of
higher level leaves in $\B_t$, and make a further split of a lower
level node, the prior will never decrease. We call this operation as
\emph{prune and split}. As the
size of $\A_t$ and $\B_t$ are the same, we can always find a pair of
leave nodes in $\B_t$ of level $\D_b$, denoted as $\Omega_{\bm
  \lambda_1, \be_1} ^{(\D_b)}$ and $\Omega_{\bm \lambda_1, \be_1+1} ^{(\D_b)}$
where $\be +1$ is understood as addition for a binary number, and a
leave node $\Omega_{\bm \lambda_2, \be_2 }^\ksup$ in $\B_t$
of level $k$ no larger than $\D_b-1$. % (\tech{Note that this leave node
  % can be an original terminal node of tree $\B_t$ or it can be the
  % merged node after the pruning step})
 Assume $\Omega_{\bm
  \lambda_1, \be_1} ^{(\D_b)}$ and $\Omega_{\bm \lambda_1, \be_1+1}
^{(\D_b)}$ are pruned and $\Omega_{\bm \lambda_2, \be_2 }^\ksup$ is
further split into two subregions, corresponding to a new binary
partition $\wt{\B}_t$ with the path $\wt{\B}_t^\1, \ldots,
\wt{\B}_t^{(\wt{\D}_b)}$, where $\wt{\D}_b = \D_b$ or $\D_b -1$. Then
\begin{eqnarray*}
  \Pi (\F_{\{\wt{\B}_t^\ksup: 1 \leq k \leq \wt{\D}_b \}})
  =
  \Pi(\F_{\treeb}) \cdot
  \frac{1-\rho_{\D_b-1}}{(1-\rho_{\D_b})^2\rho_{\D_b-1}}
  \cdot
  \frac{(1-\rho_{k+1})^2\rho_{k} }{1-\rho_{k}},
\end{eqnarray*}
since the assumption $\rho_k = c_\rho 2^{-\nu k}$ for some $\nu
>1$, it is easy to show
\begin{eqnarray*}
  \frac{(1-\rho_{\D_b-1}) (1-\rho_{k+1})^2}
  {(1-\rho_{k} )(1-\rho_{\D_b})^2} \geq 1
  \quad \mbox{and} \quad
  \frac{\rho_{k}}{\rho_{\D_b -1}} \geq 1.
\end{eqnarray*}

Another useful observation is that if for one split or several consecutive splits, different
dimensions are chosen for partitioning, the prior on the set of
random measures supported by the new partition remains the same. This
type of operation is called \emph{reshaping}.

Note that the binary partition $\A_t$ under the path $\A_t^\0,
\A_t^\1, \ldots, \A_t^{(\D_a)}$ can be obtained by applying
finite number of prune and split and reshaping operations to
$\B_t$, and these operations will \emph{not} lower the prior. 
% We may write the underlying partition alternatively as
% \begin{eqnarray*}
%   \Omega = \bigcup_{k=1}^{\D(\at)} \bigcup_{j=1}^{t_k}\Omega_{\bm \lambda_j, \be_j}^\ksup
% \end{eqnarray*}

\subsubsection{An upper bound for a balanced partition}

Next we will show if the binary partition $\A_t$ is a \emph{balanced}
size $t$ partition with path $\A_t^\0, \A_t^\1, \ldots, \A_t^{(\D)}$,
then the prior on random measures supported by it satisfies
\begin{eqnarray}
  \label{eq:priorupper}
  \Pi \l \F_{\treea} \r \leq \exp( - \lambda_1 t \log t ),
\end{eqnarray}
for some $\lambda_1 > 0$.

We first show that for the balanced tree $\T_k$ defined above,
\begin{eqnarray}
  \label{eq:priorupperbal}
  \Pi \l \F_{\treek} \r
  \leq
  \exp\l
  - \nu 2^k k \log 2  + 2^k \log c_\rho + \nu 2^{k+1} \log 2
  - 2^k \log d + 2^{k-2}\ \r
\end{eqnarray}
The proof can be finished by induction.

For $k=0$, it is easy to see that
\begin{eqnarray*}
  \Pi \l \F_{\T_0} \r = 1- \rho_0 = 1- c_\rho.
\end{eqnarray*}
We can choose the value of $c_\rho$ to make (\ref{eq:priorupperbal})
hold.

Assume the induction hypothesis hold for $k$, and the corresponding
path is $\T_k^\0, \T_k^\1, \ldots, \T_k^\ksup$. For $k+1$, assume the
first $k$ levels of the tree is the same as those of $\T_k$. Then
\begin{eqnarray*}
  \Pi \l \F_{\treeknew}\r
  &=& \Pi \l \F_{\treek} \r
  \cdot
  \prod_{\be \in\{ 0, 1 \}^k}
  \l \frac{\rho_k (1- \rho_{k+1})^2} {1 - \rho_k} \cdot \frac{1}{d} \r.
\end{eqnarray*}
By plugging in the induction hypothesis and noting that $(1-
\rho_{k+1})^2 / (1- \rho_k) \leq 1 + \frac{1}{4}\rho_k$, we have
\begin{eqnarray*}
 && \Pi \l \F_{\treeknew}\r\\
  && \hspace{0.5cm} \leq 
     \exp\l - \nu 2^k k \log 2  + 2^k \log c_\rho 
     - 2^k \log d
  + \nu 2^{k+1} \log 2+ 2^{k-2}\ \r \cdot
  \l \rho_k (1+ \rho_k /4) /d \r^{2^k} \\
  && \hspace{0.5cm} \leq \exp\Big(
     - \nu 2^k k \log 2  + 2^k \log c_\rho - 2^k \log d
  + \nu 2^{k+1} \log 2+ 2^{k-2}\ \\
     && \hspace{2cm}     + 2^k (\log c_\rho - \nu k \log 2 + \log (1+
        \rho_k /4) - \log d) \Big)\\
  && \hspace{0.5cm} \leq \exp\l
     -\nu 2^{k+1} (k+1) \log 2 + \nu 2^{k+2} \log 2
     + 2^{k+1} \log c_\rho - 2^{k+1} \log d + 2^{k-1}
     \r,
\end{eqnarray*}
where the last inequality is obtained by applying $\log ( 1+ x) \leq
x$ and $\rho_k \leq 1$. This way, we show the induction hypothesis
also holds for $k+1$.

Note that for divisions of regions in $\T_k$, if different dimensions are chosen
for the splits, the prior on random measures supported by the tree generated by a particular path
still share the same lower and upper bounds.

\subsubsection{An upper bound for $\Theta_t$}
Generally, given a size $t$, with $2^k \leq t < 2^{k+1}$
for some $k \in \mathbb{N}$, we can define a \emph{balanced} partition
$\A_t$ as
the following: first, the tree grows without stopping for the first
$k$ levels as $\T_{k+1}^\0, \T_{k+1}^\1, \ldots, \T_{k+1}^\ksup$; then
at level $k$, the split for $t-2^k$ level-$k$ regions will continue
for one more step, while the remaining $2^{k+1}- t$ ones being
stopped. The complete path for obtaining $\A_t$ is still denoted as
$\A_t^\0, \A_t^\1, \ldots, \A_t^\knew$. It is easy to see,
\begin{eqnarray*}
  \Pi \l \F_{ \{\A_t^{(l)}: 0 \leq l \leq k+1 \}} \r
  \leq
  \Pi \l \F_{\treek}\r.
\end{eqnarray*}
Applying the bound (\ref{eq:priorupperbal}) and $2^k \leq t <
2^{k+1}$, we have
\begin{eqnarray*}
  \Pi \l \F_{ \{\A_t^{(l)}: 0 \leq l \leq k+1 \}} \r
  \leq
  \exp\l
  - \frac{\nu t}{2} \log t  + t \log c_\rho + \frac{3}{2}\nu  t\log 2
  - \frac{t}{2} \log d + \frac{t}{4}  \r.
\end{eqnarray*}
As shown before, such a balanced binary partition is
preferred in the sense that (\ref{eq:preferbal}) holds. Within the
papameter space $\Theta_t$, there are at most $d^t t!$ such
paths. This is because we may consider obtaining a size $t$ partition
as the following: at each step a subregions is randomly selected for partitioning,
and for the chosen subregions the split is along the midpoint of a
randomly chosen dimension. This type of recursive partitioning is
repeated for $t-1$ steps. If we denote the decisions made at these
$t-1$ steps as $(J_1, \ldots, J_{t-1})$, then each sequence of
decisions can uniquely determine a binary partition with a specific
path. For each path, there is at least one sequence of decisions
corresponding to it. Therefore, the number of paths is bounded by the number of
different decisions, which is in turn bounded by $d^t t!$.

Combining the bounds together, we have
\begin{eqnarray}
  \label{eq:prioruppersizet}
  \nonumber \Pi \l \Theta_t \r
  &\leq&
         d^t \log t \cdot
         \exp\l
  - \frac{\nu }{2} t \log t  + t \log c_\rho + \frac{3}{2}\nu  t\log 2
  - \frac{t}{2} \log d + \frac{t}{4}  \r \\
  & \leq &
           \exp\l
  - (\nu /2-1) t \log t  + t \log c_\rho + \frac{3}{2}\nu  t\log 2
  + \frac{t}{2} \log d -\frac{3}{4} t +\log t \r.
\end{eqnarray}




==> tools/large_deviation_lower.tex <==
\subsection{Large Deviation Inequality}
 Let $\mathcal{C} = \{f \in  \Fat:
  \| f - \fat \|_\infty \leq \eta^2 \delta^2 (n, t), \tech{f \geq t (\eta^2/(2n))^{\lfloor \log_2 t \rfloor}} \}$. \tech{Note that this $\A_t$
    is usually a balanced non-stopped partition.} 
  \begin{lemma}
    \label{lemma:empineqinf}
Under the same conditions as those for \writing{Theorem
  \ref{thm:likbiasvar}}, 
\begin{eqnarray}
  \label{eq:empineqinf}
  \P_{f_0} \left(
  \inf_{f \in  \mathcal{C}}
  \sum_{i=1}^n Z_{\mathcal{A}_t, f} (Y_i)
  \leq 
   - 4n \eta^2 \delta_{n,t}^2 - n\sup_{f \in \mathcal{C}} \kl(\fat, f)
\right) 
\leq 3 \exp(-4 c_2 \eta^2 n \delta^2(n, t)).
\end{eqnarray}
  \end{lemma}
  \begin{proof}
Note that %For some unknown positive number $C$, 
\begin{eqnarray*}
 && \P_{f_0} \left(
  \inf_{f \in  \mathcal{C}}
  \sum_{i=1}^n Z_{\mathcal{A}_t, f} (Y_i)
  \leq 
   - 4 n \eta^2 \delta_{n,t}^2 -  \tech{n^{1/2}\sup_{f \in \mathcal{C}} \kl(\fat, f)}
    \right) \\
  % &&\hspace{0.5cm}
  %    \leq
  %    \P_{f_0} \left(
  % \sup_{f \in  \mathcal{C}}
  % \sum_{i=1}^n \wt{Z}_{\mathcal{A}_t, f} (Y_i)
  % \geq 
  %    n \eta^2 \delta_{n,t}^2
  %    \right) \\
  && \hspace{0.5cm}
     =
     \P_{f_0} \left(
     \inf_{f \in  \mathcal{C}}
     n^{-1/2} \sum_{i=1}^n
     \left(Z_{\mathcal{A}_t, f} (Y_i) -
     \E Z_{\mathcal{A}_t, f} (Y_i)
     +  \E Z_{\mathcal{A}_t, f} (Y_i)\right)
    \leq  -4 n^{1/2} \eta^2 \delta_{n,t}^2-\tech{n^{1/2} \sup_{f \in \mathcal{C}} \kl(\fat, f)}
     \right) \\
  && \hspace{0.5cm}
     \leq
     \P_{f_0} \left(
     \inf_{f \in  \mathcal{C}}
     n^{-1/2} \sum_{i=1}^n
     \left(Z_{\mathcal{A}_t, f} (Y_i) -
     \E Z_{\mathcal{A}_t, f} (Y_i) \right)
     \leq
     - \inf_{f \in \mathcal{C}} n^{1/2} \E Z_{\mathcal{A}_t, f} (Y_1) 
    - 4 n^{1/2} \eta^2 \delta_{n,t}^2 -\tech{n^{1/2}\sup_{f \in \mathcal{C}} \kl(\fat, f)}
     \right),
\end{eqnarray*}
where $\E Z_{\mathcal{A}_t, f} (Y_1) = - \kl (\fat, f)$ for $f \in
\Fat$. It is clear that \tech{$n^{1/2}\sup_{f \in \mathcal{C}}
  \kl(\fat, f)$} cancels with the positive term $ - \inf_{f \in
  \mathcal{C}} n^{1/2} \E Z_{\mathcal{A}_t, f} (Y_1) $. 
It suffices to bound the probability
 \begin{eqnarray*}
   && \P_{f_0} \left(
     \inf_{f \in  \mathcal{C}}
     n^{-1/2} \sum_{i=1}^n
     \left(Z_{\mathcal{A}_t, f} (Y_i) -
     \E Z_{\mathcal{A}_t, f} (Y_i) \right)
     \leq
    -4 n^{1/2} \eta^2 \delta_{n,t}^2 
      \right) \\
   && \hspace{0.5cm} =
      \P_{f_0} \left(
     \sup_{f \in  \mathcal{C}}
     n^{-1/2} \sum_{i=1}^n
     \left(- Z_{\mathcal{A}_t, f} (Y_i) +
     \E Z_{\mathcal{A}_t, f} (Y_i) \right)
     \geq 
     4 n^{1/2} \eta^2 \delta_{n,t}^2 
      \right).
 \end{eqnarray*}
 This implies that we can study the empirical process corresponding to
 $-Z_{\mathcal{A}_t, f}$. As we have assumed that the density function
 is bounded from above and below, the two empirical processes can be
 studied use similar techniques. In specific, Lemma
 \ref{lemma:largedeviation} can still be applied to the one associated
 with $-Z_{\mathcal{A}_t, f}$. Note that for any $f \in \mathcal{C}$, $\rho(f,
 \fat) \leq 2 \eta \delta(n, t)$. Consequently, the probability above is bounded by $3 \exp(-4 c_2
 \eta^2 n\delta^2(n, t))$. This finished the proof.
\end{proof}

\tech{\begin{remark}
  According to the relationship between the supnorm and the KL divergence,
  $\sup_{f \in \mathcal{C}} \kl(\fat, f) \leq 4 \eta^2
  \delta^2(n,t)$. Therefore, another way to write the inequality is 
  \begin{eqnarray}
  \label{eq:empineqinfalt}
  \P_{f_0} \left(
  \inf_{f \in  \mathcal{C}}
  \sum_{i=1}^n Z_{\mathcal{A}_t, f} (Y_i)
  \leq 
   - 8n \eta^2 \delta_{n,t}^2 
\right) 
\leq 3 \exp(-4 c_2 \eta^2 n \delta^2(n, t)).
\end{eqnarray}
\end{remark}}

We can also derive an inequality for the likelihood ratios. 
\begin{lemma}
\label{lemma:likineqinf}
  Under the same conditions as those for \writing{Theorem
  \ref{thm:likbiasvar}}, for some $\underline{c}_1 \in (0, 1), \underline{c}_2'
>0$ and the same $c_2$, 
\begin{eqnarray}
    \label{eq:likineqinf}
 \nonumber &&   \P_{f_0} \bigg( 
\inf_{f \in \mathcal{C}} 
\prod_{i=1}^n \frac{f(Y_i)}{f_0(Y_i)} 
\leq  
\exp \Big( 
-n (1+\underline{c}_1) \kl (f_0, \fat)
-4\eta^2 n \delta_{n, t}^2 
- n \sup_{f \in \mathcal{C}} \kl (\fat, f) 
\Big)
    \bigg)\\
  && \hspace{5cm}  \leq
\exp\left( -\tech{\underline{c}_2' }n \rho^2(f_0, \fat) \right)
+
    3\exp\left(-4 c_2 \eta^2 n \delta(n, t)^2 \right).
  \end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that for Theorem \ref{thm:likbiasvar}. 
We first decompose the left hand side of \eqref{eq:likineqinf}
into the following two parts:  
\begin{eqnarray*}
  \P_{f_0} \left( \inf_{f \in \mathcal{C}}
\prod_{i=1}^n \frac{f(Y_i)}{f_0(Y_i)} \leq  
\exp\Big( -n (1+\underline{c}_1) \kl (f_0, \fat)
-4\eta^2 n \delta_{n, t}^2 
- n \sup_{f \in \mathcal{C}} \kl (\fat, f) 
 \Big)\right)  \leq P_1 + P_2, 
\end{eqnarray*}
where
\begin{eqnarray*}
P_1 &=& \P \left( 
\prod_{i=1}^n \frac{\fat(Y_i)}{f_0(Y_i)}  \leq 
\exp\left( -n (1+\underline{c}_1) \kl (f_0, \fat)\right)\right), \\
  P_2 &=& \P_{f_0} \left( \inf_{f \in  \mathcal{C}}
\prod_{i=1}^n \frac{f(Y_i)}{\fat (Y_i)} \leq  
\exp \Big( 
          -4\eta^2 n \delta_{n, t}^2 
- n \sup_{f \in \mathcal{C}} \kl (\fat, f)   \Big)\right).
\end{eqnarray*}
Roughly speaking, $P_1$ cannot be too large given the approximation
ability by $\Fat$, and $P_2$ corresponds to variance. We will provide
bounds for these two terms separately.

By Lemma \ref{lemma:empineqinf}, we know
\begin{eqnarray*}
  P_2 \leq 3 \exp\left( -4 c_2 \eta^2 n \delta_{n, t}^2 \right).
\end{eqnarray*}

In order to bound $P_1$, we would like to apply the Bernstein's
inequality. Let $Z_{\fat} = \fat/ f_0$, 
\begin{eqnarray*}
  P_1 = \P \left( \sum_{i=1}^n \left( {Z}_{\fat}(Y_i) 
  - \E {Z}_{\fat}(Y_i)\right)
  \leq 
  - (1+\underline{c}_1) n \kl (f_0, \fat)- n \E {Z}_{\fat} (Y_1)
  \right).
\end{eqnarray*}
% By \writing{Lemma ??}, 
As $- \E {Z}_{\fat} (Y_1) = \kl ( f_0, \fat) % \leq
% c_{\mbox{\scriptsize{kl}}}\rho^2(f_0, \fat)
$, 
% \tech{where $c_{\mbox{\scriptsize{kl}}}$ is a constant
% depending on the boundedness of $f_0$.} Plugging in this bound for
% the truncated log-likelihood ratio, we have
we can rewrite $P_1$ as 
\begin{eqnarray*}
  P_1 =  \P \left( n^{-1/2}\sum_{i=1}^n \left( {Z}_{\fat}(Y_i) 
  - \E {Z}_{\fat}(Y_i)\right)
  \leq 
 - \underline{c}_1 n^{1/2} \kl (f_0, \fat) 
  \right).
\end{eqnarray*}
% With appropriately chosen $\underline{c}_1$, we may assume
% $(1+\underline{c}_1-c_{\mbox{\scriptsize{kl}}})>0$. 
\tech{To apply the Bernstein's inequality, we need the moment of
  $Z_{\fat}$ to be bounded. Then $\fat / f_0$ can not be too
  large. $f_0$ needs to be bounded from below.}
Then by the Bernstein's inequality, with \tech{some $c_0 = (\exp(\tau/2) -1 -
\tau/2)/(1- \exp(-\tau/2))^2$}, we obtain
% \begin{eqnarray*}
%  % \label{eq:P2bound}
%  \nonumber  P_1 &\leq& 
% \exp\left( 
% - \frac{(1+\underline{c}_1-c_{\mbox{\scriptsize{kl}}})^2 n \rho^4(f_0, \fat) }
%   {8 \left( 8c_0 \rho^2(f_0, \fat)  
% + 2  (1+\underline{c}_1-c_{\mbox{\scriptsize{kl}}})\rho^2(f_0,\fat) \right)}\right)\\
%   &\leq& \exp\left(
% - \frac{(1+\underline{c}_1-c_{\mbox{\scriptsize{kl}}})^2}
% {(2^6c_0 +2^4 (1+\underline{c}_1-c_{\mbox{\scriptsize{kl}}}))}
%   \cdot n \rho^2(f_0, \fat)\right).
% \end{eqnarray*}
\begin{eqnarray*}
 % \label{eq:P2bound}
 \nonumber  P_1 &\leq& 
\exp\left( 
- \frac{(\underline{c}_1)^2 n \kl^2 (f_0, \fat) }
  {8 \left( 8c_0 \rho^2(f_0, \fat)  
+ 2  \underline{c}_1 \kl (f_0,\fat) \right)}\right)\\
  &\leq& \exp\left(
- \frac{(\underline{c}_1)^2}
{2^6c_0 +2^4 \underline{c}_1}
  \cdot n  \kl (f_0, \fat)\right).
\end{eqnarray*}

Finally, the desired result follows the upper bounds for $P_1$ and $P_2$.
\end{proof}

% For this term
%  \begin{eqnarray*}
%    - \inf_{f \in \mathcal{C}} n^{1/2} \E Z_{\mathcal{A}_t, f} (Y_1)
%    = n^{1/2} \sup_{f \in \mathcal{C}} \left( - \E Z_{\mathcal{A}_t, f} (Y_1) \right)
%    =n^{1/2} \sup_{f \in \mathcal{C}} \kl(\fat, f). 
%  \end{eqnarray*}
%  Therefore
%  \begin{eqnarray*}
%    C = n^{1/2} \sup_{f \in \mathcal{C}} \kl(\fat, f)
%    \quad
%    \mbox{and}
%    \quad
%     \sup_{f \in \mathcal{C}} \kl(\fat, f) \leq b \eta^2 \delta_{n,t}^2
%    \left( \log (\eta \delta_{n, t})^{-1} \right)^2.
%  \end{eqnarray*}
%  % As $\rho^2(\fat, f) \leq \kl (\fat, f).$
%  In the case the density functions are bounded from above and below,
%  \begin{eqnarray*}
%     C = n^{1/2} \sup_{f \in \mathcal{C}} \kl(\fat, f)
%    \quad
%    \mbox{and}
%    \quad
%     \sup_{f \in \mathcal{C}} \kl(\fat, f) \leq b \eta^2 \delta_{n,t}^2.
%  \end{eqnarray*}

 \subsubsection*{Bernstein's Inequality}
 \begin{lemma}[Bernstein's inequality]
   Let $Y_1, \ldots, Y_n$ be independent random variables with zero mean such that $E|Y_i|^m \leq m ! b^{m-2} v/2$, for every $m \geq 2$ and some constants $b$ and $v$. Then
   \begin{eqnarray*}
     && \P( \sum_{i=1}^n Y_i \geq t ) \leq \exp (-\frac{t^2/2}{nv + b t})
        \quad \mbox{or} \quad
        \P( n^{-1/2}\sum_{i=1}^n Y_i \geq \epsilon )
        \leq
        \exp (-\frac{\epsilon^2n/2}{nv + b \epsilon n^{1/2}}), \\
     &&\P( \sum_{i=1}^n Y_i \leq- t ) \leq \exp (-\frac{t^2/2}{nv + b t})
        \quad \mbox{or} \quad
        \P( n^{-1/2}\sum_{i=1}^n Y_i \leq - \epsilon )
        \leq
        \exp (-\frac{\epsilon^2/2}{v + b \epsilon /n^{1/2}}) .
   \end{eqnarray*}
 \end{lemma}
 In the lemma, the Bernstein's condition is imposed on central moments. If we assume for non-central moments
 \begin{eqnarray*}
   E|Y_i|^m \leq m ! b^{m-2} v/2.
 \end{eqnarray*}
 Then
 \begin{eqnarray*}
   E| Y_i - EY_i|^m \leq E (|Y_i| + E|Y_i|)^m \leq 2^{m-1}\E (|Y_i|^m + (E|Y_i|)^m) \leq 2^m E|Y_i|^m \leq m! (2b)^{m-2} (4v)/2.
 \end{eqnarray*}
 This implies that for central moments, the condition is satisfied with $b' = 2b$ and $v' = 4v$. Plugging in $b'$ and $v'$, we obtain a form of Bernstein's inequality consistent with the one in the paper by Wong and Shen (1995).

 For Bernstein's condition on non-central moments, the previous result can be further improved, which is summarized below.
 \begin{lemma}[Bernstein's inequality with non-central moment condition]
   Let $Y_1, \ldots, Y_n$ be independent random variables such that $E|Y_i|^m \leq m ! b^{m-2} v/2$, for every $m \geq 2$ and some constants $b$ and $v$. Then
   \begin{eqnarray*}
     && \P( \sum_{i=1}^n( Y_i - \E Y_i)  \geq t ) \leq \exp (-\frac{t^2/2}{nv + b t})
        \quad \mbox{or} \quad
        \P( n^{-1/2}\sum_{i=1}^n (Y_i - \E Y_i) \geq \epsilon )
        \leq
        \exp (-\frac{\epsilon^2n/2}{nv + b \epsilon n^{1/2}}), \\
     &&\P( \sum_{i=1}^n (Y_i - \E Y_i)  \leq- t ) \leq \exp (-\frac{t^2/2}{nv + b t})
        \quad \mbox{or} \quad
        \P( n^{-1/2}\sum_{i=1}^n (Y_i - \E Y_i)  \leq - \epsilon )
        \leq
        \exp (-\frac{\epsilon^2n /2}{n v + b \epsilon n^{1/2}}) .
   \end{eqnarray*}
 \end{lemma}

%  For the truncated log-likelihood ratios, we still have the following result
%  \begin{eqnarray*}
%    \P \left(
%    n^{-1/2} \sum_{i=1}^n
%    \left(\wt{Z}_f (Y_i) - \E \wt{Z}_f \right) \leq - t \right)
%    \leq
%    \exp \left(
%    - \frac{t^2}
%    {8(8c_0 \rho^2(f, f_0) + 2t/ n^{1/2})}\right),
%  \end{eqnarray*}
%  for any $t>0$. $c_0$ can be chosen as $(\exp(\tau/2) - 1 - \tau/2)/(1 - \exp(-\tau/2))^2$.

%  \subsubsection*{Large-Deviation Inequality}
%  To obtain the large-deviation inequality along the other direction,
%  we may use a trick. It suffices to bound the probability
%  \begin{eqnarray*}
%    && \P_{f_0} \left(
%      \inf_{f \in  \mathcal{C}}
%      n^{-1/2} \sum_{i=1}^n
%      \left(Z_{\mathcal{A}_t, f} (Y_i) -
%      \E Z_{\mathcal{A}_t, f} (Y_i) \right)
%      \leq
%     - n^{1/2} \eta^2 \delta_{n,t}^2 
%       \right) \\
%    && \hspace{0.5cm} =
%       \P_{f_0} \left(
%      \sup_{f \in  \mathcal{C}}
%      n^{-1/2} \sum_{i=1}^n
%      \left(- Z_{\mathcal{A}_t, f} (Y_i) +
%      \E Z_{\mathcal{A}_t, f} (Y_i) \right)
%      \geq 
%      n^{1/2} \eta^2 \delta_{n,t}^2 
%       \right).
%  \end{eqnarray*}
%  This implies that we can study the empirical process corresponding to
%  $-Z_{\mathcal{A}_t, f}$. As we have assumed that the density function
%  is bounded from above and below, the two empirical processes can be
%  studied use similar techniques. In specific, Lemma
%  \ref{lemma:largedeviation} can still be applied to the one associated
%  with $-Z_{\mathcal{A}_t, f}$. Therefore,
%  \begin{eqnarray*}
%     \P_{f_0} \left(
%      \sup_{f \in  \mathcal{C}}
%      n^{-1/2} \sum_{i=1}^n
%      \left(- Z_{\mathcal{A}_t, f} (Y_i) +
%      \E Z_{\mathcal{A}_t, f} (Y_i) \right)
%      \geq 
%      n^{1/2} \eta^2 \delta_{n,t}^2 
%       \right) \leq 3 \exp(-c_2 \eta^2 n \delta_{n, t}^2).
%  \end{eqnarray*}
%  In summary, for the likelihood ratio,
%  \begin{eqnarray*}
%    \P_{f_0} \left(\inf_{f \in \mathcal{C}} \sum_{i=1}^n
%    Z_{\mathcal{A}_t, f} (Y_i) \leq -n \eta^2 \delta_{n, t}^2 - b'
%    \eta^2 n \delta_{n, t}^2 \left( \log (\eta \delta_{n, t})^{-1} \right)^2 \right)
%    \leq 3 \exp(-c_2 \eta^2 n \delta_{n, t}^2).
%  \end{eqnarray*}
%  Or
%  \begin{eqnarray*}
%    \P_{f_0} \left(\inf_{f \in \mathcal{C}} \sum_{i=1}^n
%    Z_{\mathcal{A}_t, f} (Y_i) \leq -2 b'
%    \eta^2 n \delta_{n, t}^2 \left( \log (\eta  \delta_{n, t})^{-1} \right)^2\right)
%    \leq
%    3 \exp\left(-c_2 b'^2 \eta^2 n \delta_{n, t}^2
%    \left( \log (\eta \delta_{n, t})^{-1} \right)^2 \right).
%  \end{eqnarray*}
%  In the case the density functions are bounded from above and below,
%  \begin{eqnarray*}
%    \P_{f_0} \left(\inf_{f \in \mathcal{C}} \sum_{i=1}^n
%    Z_{\mathcal{A}_t, f} (Y_i) \leq - (1+b)
%    \eta^2 n \delta_{n, t}^2 \right)
%    \leq
%    3 \exp\left(-c_2 \eta^2 n \delta_{n, t}^2 \right).
%  \end{eqnarray*}
%  Or equivalently
%  \begin{eqnarray*}
%    \P_{f_0} \left(\inf_{f \in \mathcal{C}} \sum_{i=1}^n
%    Z_{\mathcal{A}_t, f} (Y_i) \leq
%    -  \eta^2 n \delta_{n, t}^2 \right)
%    \leq
%    3 \exp\left(-c_2' \eta^2 n \delta_{n, t}^2 \right).
%  \end{eqnarray*}
